Type Annotation for Adaptive Systems

We introduce type annotations as a flexible typing mechanism for graph systems and discuss their advantages with respect to classical typing based on graph morphisms. In this approach the type system is incorporated with the graph and elements can adapt to changes in context by changing their type annotations. We discuss some case studies in which this mechanism is relevant.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Alexander Heu{\ss}ner, Aleks Kissinger, Anton Wijs (Eds.):\\ 2nd Graphs as Models workshop (GaM 2016)\\
EPTCS 231, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.231.1}{10.4204/EPTCS.231.1}}
\pdfoutput=1

